Network Friendly Recommendations: Optimizing for Long Viewing Sessions

Caching algorithms try to predict content popularity, and place the content closer to the users. Additionally, nowadays requests are increasingly driven by recommendation systems (RS). These important trends, point to the following: \emph{make RSs favor locally cached content}, this way operators reduce network costs, and users get better streaming rates. Nevertheless, this process should preserve the quality of the recommendations (QoR). In this work, we propose a Markov Chain model for a stochastic, recommendation-driven \emph{sequence} of requests, and formulate the problem of selecting high quality recommendations that minimize the network cost \emph{in the long run}. While the original optimization problem is non-convex, it can be convexified through a series of transformations. Moreover, we extend our framework for users who show preference in some positions of the recommendations' list. To our best knowledge, this is the first work to provide an optimal polynomial-time algorithm for these problems. Finally, testing our algorithms on real datasets suggests significant potential, e.g., $2\times$ improvement compared to baseline recommendations, and 80\% compared to a greedy network-friendly-RS (which optimizes the cost for I.I.D. requests), while preserving at least 90\% of the original QoR. Finally, we show that taking position preference into account leads to additional performance gains.

==> fast_myopic.tex <==
%\begin{comment}-One approach is to solve the easier problem of finding the single step cache friendly recommendations. 
%Present it and discuss the problem (it is LP and can be solved with the use of a commercial solver).\end{comment}

In the previous section, we have presented an efficient iterative algorithm that is guaranteed to converge to the optimal cache-friendly recommendations in polynomial time. Nevertheless, when the content catalogue is large (e.g., more than 10K contents) this algorithm might not scale well as it would have to deal with 100 million variables. In such scenarios one might reasonably opt for a suboptimal solution to the problem, that can at least be obtained in reasonable time. The following algorithm does so, by considering only the first Markovian step in a user session, and greedily optimizing for it (i.e., not considering subsequent steps).


%Having defined the hard problem of multistep vision recommendations in the section \ref{sec:problem_formulation}, one would plausibly wonder \textit{how about solving the significantly easier problem of 1-step vision recommender?} 

Minimizing the cost of content retrieval in one step of a Markovian transition is equivalent to minimize the scalar quantity $f(\mathbf{R}) = \mathbf{p}_0^{T} \cdot(\frac{a}{N}\cdot\mathbf{R}+(1-a) \cdot \mathbf{P}) \cdot \mathbf{c}$. As only the first term of $f(\mathbf{R})$ depends on the control variable $\mathbf{R}$, the second term could be ignored, giving rise to the problem of minimizing the content retrieval cost with the help of Greedy Cache-Friendly Recommendations (GCFR).%from the process of optimization. As a consequence the problem of minimizing the content retrieval cost with the help of Greedy Cache-Friendly Recommendations (GCFR) may be written as follows.
%\begin{problem}[Greedy Cache-Friendly Recommendations]\label{problem:myopic}
\begin{small} 
\begin{align} 
\underset{\mathbf{R}}{\mbox{minimize}}~~ \; & 
\mathbf{p}_0^{T} \cdot \mathbf{R} \cdot \mathbf{c},\\
s.t.~~~ &\text{Eqs. (\ref{affine-con})--(\ref{box-con})} \label{constraint-set-myopic}
\end{align}
\end{small}
%\end{problem}
The above problem is again an LP, and can be tackled with commercial solvers, as discussed earlier. 
%The \probref{problem:myopic} is a Linear Program (LP) and can be solved in polynomial time with the use of efficient commercial solvers (GUROBI, MOSEK etc) that run interior-point methods or SIMPLEX. Unfortunately, since our problem contains millions of variables or more, even well established solvers could take some time to return the solution. 
Interestingly, when the cost values $\mathbf{c}$ are binary and the utility weights $u_{ij}$ are generic (or the utility weights are binary and the cost values generic), then the problem can be solved with a much faster customized algorithm.
%Interestingly in some cases, the problem is well structured, and simply plugging it to an LP solver will be a procedure slower than necessary.
The following lemma solves the problem for generic cost (e.g., hierarchical caching) and binary $u_{ij}$ values (either strongly related iterms or not related at all)
%We consider the case which corresponds to hierarchical caching, i.e when the cost vector is generic We further assume that $u_{ij}$ are 0-1, corresponding to the case of genuinely good or bad recommendations.
%For the case where the both these quantities are binary we propose the following fast algorithm.% of $O(K^2)$ complexity that resolves the single step recommendations.

%\theo{The algorithm as written here, is the simplest version which solves the problem when the cost vector and the utility weights are both binary}

%\todo{For the final version this has to be updated to solve the case where at least one entity is generic and the other is binary}
%\begin{algorithm} 
%\begin{algorithmic} [1]
%\caption{Fast Myopic (FM)}\label{alg:myopic}
%\Statex {Input: N, $\mathbf{U}$, q, $\mathbf{c}$} \Comment (system parameters)
%\State $\mathcal{C} =$ order($\mathbf{c}$) ($c_1 < c_2 <...< c_K$)
%\For{i = 1,...,K}
%\State {$\mathcal{S}_{i}=$ order($\mathcal{C} \cap \mathcal{U}_{i}$)}
%\State budget $\gets N$
%\While {$q \ge 0 or budget \ge 0$}
%\State {$r_{ij} \gets \min\{1,q\}~\forall j \in \mathcal{S}_{i}$}
%\State budget $\gets$ budget $- r_{ij}$
%\EndWhile
%\While budget $\ge 0$
%'b
%\EndWhile
%\State $r_{ij} \gets 1~ \forall j \in \mathcal{S}_{i}$
%\State $q_{rem} = q - q_{\mathcal{S}_{i}}$
%\State budget $= N - \sum_{j} R_{ij}$
%\If {$q_{rem} > 0$}
%\While {$q_{rem} > 0$}
%\State $r_{ij} \gets 1~$ for a $j \in \mathcal{U}_{i}$
%\State Update budget
%\EndWhile
%\Else
%\State Assign leftover budget to contents in $\mathcal{C}$
%\EndIf
%\While budget $\ge 0$
%\State blah blaj
%\EndWhile
%\EndFor
%\State $return~~R$
%\end{algorithmic}
%\end{algorithm}

\begin{lemma} \label{greedy-method}
When $c_i \in \mathbb{R}$ and $u_{ij} \in\{0,1\}$ the optimal solution of GCFR is obtained as follows. For each content $i$, we list the related items in increasing cost. We choose $r_{ij} = 1$ for each of them until the quality constraint is satisfied. If $q$ is multiple of $N$ then these $r_{ij}$ will be all 1's. Otherwise there will be one $r_{il} < 1$. Once $q$ is satisfied, we assign $r_{ij} = 1$ to the least cost contents available, and assign this remaining $1-r_{il}$ to the least cost content not recommended yet.
\end{lemma}

\begin{proof}
The function $f(\mathbf{R}): \mathbb{R}^{K \times K} \rightarrow \mathbb{R}$ can be written as $f(\mathbf{R})= \mathbf{p}_0^{T}\cdot \mathbf{R} \cdot \mathbf{c} = \sum_{i \in \mathcal{K}} p_{0}^{i} \sum_{j \in \mathcal{K}} r_{ij} c_{j}$. Note that the quantity inside the second summation contains the matrix $\mathbf{R}$ rows, exactly like the set of constraints described in \ref{constraint-set-myopic}.
Based on the fact that $\min_{\mathbf{R}} f(\mathbf{R}) = \min_{\mathbf{R}} \sum_{i \in \mathcal{K}} f_{i}(\mathbf{R}_{i|\cdot}) = \sum_{i \in \mathcal{K}} \min_{\mathbf{R}{i|\cdot}} f_{i}(\mathbf{R}_{i|\cdot})$.
Each of these $K$ problems can be treated independently. 
The method of Lemma~\ref{greedy-method} finds the optimal for the GCFR as any other feasible solution will satisfy the quality constraint with higher cost contents.
\end{proof}

We present two tables, one showing the tradeoff of greedy myopic, LP-MOSEK myopic and ADMM in terms of optimizing Opt~\ref{problem:basis} and execution time for a synthetic scenario ($C/K = 0.8\%, N=2, Q = 90\%, s = 0.5~\text{(zipf exponent)}$) for a library of 1K contents, and a second one capturing only the execution time of LP-myopic and Greedy Myopic. Table~\ref{table:lp-myopic-lp-greedy-admm-comparison}, shows the immense improvement we get in terms performance with a reasonable execution time when using ADMM, while Table~\ref{table:myopic-mosek-comparison} shows it is preferable to solve GCFR with the method of Lemma~\ref{greedy-method} than simply plugging it in a generic solver.

\begin{table}
\centering
\caption{LP-Myopic vs Greedy-Myopic vs ADMM}\label{table:lp-myopic-lp-greedy-admm-comparison}
\begin{small}
\begin{tabular}{l|l|l|l}
%\hline
{}						&{LP-MOSEK} &{Greedy} &{ADMM}\\
\hline \hline
{Performance (\%)}			&{11.13} &{11.17} &{21.51}\\
\hline
{Execution time (sec)}			&{140.58} &{0.09} &{553.19}\\
\hline

\end{tabular}
\end{small}
\end{table}


\begin{table} 
\centering 
\caption{Execution times (sec) vs Library size \theo{a bit redundant I think}}\label{table:myopic-mosek-comparison}
\begin{small}
\begin{tabular}{l|l|l|l}
%\hline
{}						&{200} &{1000} &{2000}\\
\hline \hline
{LP-mosek}				&{1.1668} &{130.039} &{1137.2}\\
\hline
{MyopicAlgo}			&{0.0556} &{0.1418} &{0.3987}\\
\hline

\end{tabular}
\end{small}
\end{table}

==> fast_myopic_and_hybrid__pavlos.tex <==
%\pavlos{I do major changes in this section. I write the new version in the file ``fast\_myopic\_and\_hybrid\_\_pavlos.tex''.}

In the previous section, we designed an efficient iterative algorithm that is guaranteed to converge to the optimal cache-friendly recommendations. Nevertheless, the optimization problem comprises $\mathcal{O}(K^{2})$ variables $r_{ij}$. Hence, in some practical scenarios, applying \emph{ALGO-Main} can be challenging, or it might be desired to obtain recommendations timely, even at the cost of a suboptimal solution. To this end, in this section we design a heuristic algorithm (Section~\ref{sec:hybrid}) that is based on (i) the optimal \emph{ALGO-Main} and (ii) a very lightweight algorithm that solves a simplified version of the original problem \textbf{Opt~\ref{problem:basis}} (Section~\ref{sec:greedy}).


\subsection{Single-Step Per-Content Optimization}\label{sec:greedy}
We first present Algorithm~\ref{alg:greedy} (\textit{Greedy}), which we later use as a building block of our heuristic algorithm. \textit{Greedy} considers a \say{single-content session} (similarly to the approaches of~\cite{chatzieleftheriou2017caching,sermpezis2018soft}), and optimizes recommendations for it.



%Having defined the hard problem of multistep vision recommendations in the section \ref{sec:problem_formulation}, one would plausibly wonder \textit{how about solving the significantly easier problem of 1-step vision recommender?} 

Minimizing the cost of content retrieval in a single-content session (i.e., only one transition in the Markov chain) is equivalent to minimizing the scalar quantity $\mathbf{p}_0^{T} \cdot(\frac{a}{N}\cdot\mathbf{R}+(1-a) \cdot \mathbf{1}^{T} \cdot \mathbf{p}_{0}) \cdot \mathbf{c}$. Ignoring the terms that do not depend on the control variable $\mathbf{R}$, gives rise to the Greedy Cache Friendly Recommendations (GCFR).
%Minimizing the cost of content retrieval in a one step of a Markovian transition is equivalent to minimize the scalar quantity $f(\mathbf{R}) = \mathbf{p}_0^{T} \cdot(\frac{a}{N}\cdot\mathbf{R}+(1-a) \cdot \mathbf{P}) \cdot \mathbf{c}$. As only the first term of $f(\mathbf{R})$ depends on the control variable $\mathbf{R}$, the second term could be ignored, giving rise to the problem of minimizing the content retrieval cost with the help of Greedy Cache-Friendly Recommendations (GCFR).%from the process of optimization. As a consequence the problem of minimizing the content retrieval cost with the help of Greedy Cache-Friendly Recommendations (GCFR) may be written as follows.
\begin{subequations}\label{eq:single-step-LP}
\begin{align} 
\underset{\mathbf{R}}{\mbox{minimize}}~~ \; & 
\mathbf{p}_0^{T} \cdot \mathbf{R} \cdot \mathbf{c},\tag{\ref{eq:single-step-LP}}\\
s.t.~~~ &\text{Eqs. (\ref{quality-con})--(\ref{box-con})} \label{constraint-set-myopic}
\end{align}
\end{subequations}

Unlike the multi-step problem, this is already an LP, and can be solved directly without the earlier transformation steps; it can be tackled with commercial solvers, as discussed earlier. 
%The \probref{problem:myopic} is a Linear Program (LP) and can be solved in polynomial time with the use of efficient commercial solvers (GUROBI, MOSEK etc) that run interior-point methods or SIMPLEX. Unfortunately, since our problem contains millions of variables or more, even well established solvers could take some time to return the solution. 
Interestingly, when the cost values $\mathbf{c}$ are generic and the similarity scores $u_{ij}$ are binary, then applying \textit{Greedy} for each content separately, solves the problem much faster.
%Interestingly in some cases, the problem is well structured, and simply plugging it to an LP solver will be a procedure slower than necessary.
The following lemma proves this for generic cost (e.g., hierarchical caching) and binary $u_{ij}$ values (i.e., only strongly related $u_{ij}=1$ or unrelated $u_{ij}=0$ items exist).
%We consider the case which corresponds to hierarchical caching, i.e when the cost vector is generic We further assume that $u_{ij}$ are 0-1, corresponding to the case of genuinely good or bad recommendations.
%For the case where the both these quantities are binary we propose the following fast algorithm.% of $O(K^2)$ complexity that resolves the single step recommendations.

%\theo{The algorithm as written here, is the simplest version which solves the problem when the cost vector and the utility weights are both binary}

%\todo{For the final version this has to be updated to solve the case where at least one entity is generic and the other is binary}
%\begin{algorithm} 
%\begin{algorithmic} [1]
%\caption{Fast Myopic (FM)}\label{alg:myopic}
%\Statex {Input: N, $\mathbf{U}$, q, $\mathbf{c}$} \Comment (system parameters)
%\State $\mathcal{C} =$ order($\mathbf{c}$) ($c_1 < c_2 <...< c_K$)
%\For{i = 1,...,K}
%\State {$\mathcal{S}_{i}=$ order($\mathcal{C} \cap \mathcal{U}_{i}$)}
%\State budget $\gets N$
%\While {$q \ge 0 or budget \ge 0$}
%\State {$r_{ij} \gets \min\{1,q\}~\forall j \in \mathcal{S}_{i}$}
%\State budget $\gets$ budget $- r_{ij}$
%\EndWhile
%\While budget $\ge 0$
%'b
%\EndWhile
%\State $r_{ij} \gets 1~ \forall j \in \mathcal{S}_{i}$
%\State $q_{rem} = q - q_{\mathcal{S}_{i}}$
%\State budget $= N - \sum_{j} R_{ij}$
%\If {$q_{rem} > 0$}
%\While {$q_{rem} > 0$}
%\State $r_{ij} \gets 1~$ for a $j \in \mathcal{U}_{i}$
%\State Update budget
%\EndWhile
%\Else
%\State Assign leftover budget to contents in $\mathcal{C}$
%\EndIf
%\While budget $\ge 0$
%\State blah blaj
%\EndWhile
%\EndFor
%\State $return~~R$
%\end{algorithmic}
%\end{algorithm}

\begin{lemma} \label{greedy-method}
When $c_i \in \mathbb{R}$ and $u_{ij} \in\{0,1\}$ the optimal solution of \eq{eq:single-step-LP} is obtained by applying Algorithm~\ref{alg:greedy} $\forall i \in\mathcal{K}$.
\end{lemma}

\vspace{5pt}
\begin{algorithm}[h]
\begin{small}
\begin{algorithmic} [1]
\caption{Greedy}\label{alg:greedy}
\Statex {Input: $i, N, q, q_{i}^{max}, \mathbf{U}, \mathbf{c}$}
\State $R_{i}\leftarrow \emptyset$ \Comment set of recommendations for $i$
\State $current\_q\leftarrow 0$
\State $S_{1}\leftarrow \textproc{SortByIncreasingCost}\left(\{j\in\mathcal{K}: u_{ij}=1\}, \mathbf{c}\right)$
\While{$(current\_q < q\cdot q_{i}^{max})$ and $(|R_{i}|<N)$}
	\State $j\leftarrow \textproc{GetNextItem}(S_{1})$
	\State $R_{i}\leftarrow R_{i}\cup \{j\}$
    \State $current\_q\leftarrow current\_q+u_{ij}$
\EndWhile
\State $S_{2}\leftarrow \textproc{SortByIncreasingCost}\left(\mathcal{K}\backslash R_{i}, \mathbf{c}\right)$
\While{$|R_{i}|<N$}
	\State $j\leftarrow \textproc{GetNextItem}(S_{2})$
	\State $R_{i}\leftarrow R_{i}\cup \{j\}$
\EndWhile
\State\Return $R_{i}$
\end{algorithmic}
\end{small}
\end{algorithm}
% \vspace{5pt}
% \begin{lemma} \label{greedy-method}
% The greedy algorithm described in Algorithm 2 returns the optimal solution for the Single-Access cache friendly recommendation.
% \end{lemma}

\begin{proof}
%The proof can be found in the Technical report.
We denote our single step cost function (see Eq.(\ref{eq:single-step-LP})) as $f(\mathbf{R})=\mathbf{p}_0^{T} \cdot \mathbf{R} \cdot \mathbf{c}: \mathbb{R}^{K \times K} \rightarrow \mathbb{R}$ and the $i$-th row of $\mathbf{R}$ as $\mathbf{R}_i$ (a row vector). Then
\begin{equation}
f(\mathbf{R})= \sum_{i=1}^{K} p_{0}^{i} \sum_{j=1}^{K} r_{ij}\cdot c_{j} = \sum_{i=1}^{K} p_{0}^{i} \cdot (\mathbf{R}_i \cdot \mathbf{c}). 
\end{equation}
Note that the quantity inside the second summation (over $j$) contains only the matrix $\mathbf{R}$ rows. Importantly observe that the problem \emph{does not} have any constraint that couples different rows of $\mathbf{R}$ (\eq{constraint-set-myopic}). Using the above, we can write
\begin{align}
\min_{\mathbf{R}} f(\mathbf{R}) = \min_{\mathbf{R}_1,...,\mathbf{R}_K} \sum_{i=1}^{K}p_0^{i}\cdot (\mathbf{R}_i \cdot \mathbf{c})= \\ \nonumber \min_{\mathbf{R}_1,...,\mathbf{R}_K} \sum_{i=1}^{K} p_0^{i}\cdot (\mathbf{R}_i \cdot \mathbf{c}) = 
 p_0^{i} \sum_{i=1}^{K} \min_{\mathbf{R}_i} (\mathbf{R}_i \cdot \mathbf{c}).
\end{align}
Hence, the problem can be solved, by solving the sub-problems for each content independently. In the following we show that Algorithm~2 is optimal for each sub-problem.
% After that step, we focus on why the greedy per-content recommendation algorithm is optimal for each respective minimization. 

We denote the set of contents that constitute the whole library as $\mathcal{K}$ and the set of related contents for item $i$ as $\mathcal{U}_i$. The latter set is essential as \emph{only} the contents coming from it can satisfy the quality constraint Eq.(\ref{quality-con}).
% The problem has to primarily obey the box constraints, $0\le r_{ij}\le 1$ and further two additional constraints, Eqs.(\ref{quality-con},\ref{affine-con}). 
To obtain a feasible solution, we need to recommend contents from $\mathcal{U}_{i}$ until Eq.(\ref{quality-con}) is satisfied, and then consider any other content (if needed).%For a feasible solution we focus initially on Eq.(\ref{quality-con}), $\mathcal{U}_i$, and discard the rest of the contents as they cannot help in satisfying that specific constraint. 
 Importantly, since \emph{all contents in $\mathcal{U}_i$ contribute equally} to the constraint (i.e., $u_{ij}=1, \forall j\in \mathcal{U}_{i}$), recommending \emph{any} of them has the same effect to the total quality that needs to satisfy the constraint of  Eq.(\ref{quality-con}).% we can pick, \emph{whichever} ones we want. 
Hence, it is straightforward to see that by recommending 1-by-1 the ones with the lowest costs (and assigning $r_{ij}=1$) leads to the less total cost% We proceed by picking one-by-one the ones with the lowest cost (assigning full per content budget $r_{ij}=1$)
; doing otherwise would produce a feasible but higher cost selection, and thus would be suboptimal. 
Let us denote as $\mathcal{R}_i$ the minimum set of recommendations from $\mathcal{U}_{i}$ that satisfy the constraint of Eq.(\ref{quality-con}). %In doing so, we have created a collection of contents, which we denote as $\mathcal{R}_i$. 
If there are less than $N$ contents in $\mathcal{R}_i$, then this means that $N-|\mathcal{R}_i|$ more recommendations are needed. However, now \emph{any} content can be recommended (since Eq.(\ref{quality-con}) is already satisfied by the contents in $\mathcal{R}_i$). Hence, the optimal solution is to select the $N-|\mathcal{R}_i|$ contents with the lowest costs; any other selection would produce a higher total cost. %If there is any budget left, i.e. ($N- q \cdot q_i^{max}$), we sort again the contents of the set $\mathcal{K} \setminus \mathcal{R}_i$, and pick the ones of least cost in the same fashion as earlier, this will complete the set of recommended contents $\mathcal{R}_i$ with the least cost possible, any other selection would produce higher cost.
%
% Regarding the quality constraint, we can set the inequality to equality and combine it with the box constraint; this will yield a generalized simplex constraint over the variables of $\mathcal{U}_i$ as follows $\mathcal{Q}_i = \{ r_{ij}: \sum_{\mathcal{U}_i} r_{ij} = q~ \text{and}~ 0\le r_{ij}\le 1 \}$. 
% \begin{proposition}
% Selecting greedily the variables of lowest cost one-by-one and assigning $r_{ij}=1$, returns a solution for the subset of items in $\mathcal{U}_i$ that is also $\in \mathcal{Q}_i$ with the optimal cost. For proof see Appendix B.
% \end{proposition}
% There are in total $\binom{|\mathcal{U}_i|}{\floor{q}}$
% If we remove the quality constraint from the problem, then the optimal solution is simply \say{pick the $N$ least cost items and assign the maximum allowable value ($r_{ij}$ = 1)}. Putting the constraint back, we can see that when $u_{ij} \in [0,1]$, the problem is clearly an LP. However, if we restrict our attention to the case where $u_{ij} \in\{0,1\}$, all items contribute the \emph{equally} in terms of the quality constraint. So we list the related items in increasing cost and then choose $r_{ij} = 1$ for each of them until the quality constraint is satisfied. If $q$ is multiple of $N$ then these $r_{ij}$ will be all 1's. Otherwise there will be one $r_{il} < 1$. Once $q$ is satisfied, we assign $r_{ij} = 1$ to the least cost contents available, and assign this remaining $1-r_{il}$ to the least cost content not recommended yet.
\end{proof}

 
% Algorithm~\ref{alg:greedy} finds the optimal for the problem \eq{eq:single-step-LP} as any other feasible solution will satisfy the quality constraint with higher cost contents.\pavlos{this last sentence is not a proof, but only an unsupported statement}
% \end{proof}


To highlight the lightweight nature of \textit{Greedy}, we compare it against the \emph{ALGO-Main}, as well as with an implementation in the MOSEK software that solves the LP problem Eq.(\ref{eq:single-step-LP}) (\textit{LP-MOSEK}). In Table~\ref{table:lp-myopic-lp-greedy-admm-comparison}, we present results for the performance in term of \emph{cache hit rate} and execution time for a catalog of $K=1000$ contents (synthetic scenario, with cache size/catalog size $C/K$=0.8\%,~$N$=2,~$q$=90\%,~$s$=0.5). Observe that \emph{ALGO-Main} outperforms the two \emph{Greedy} routines by $2\times$, in terms of hit rate. However, the execution time of the latter is lower. More importantly the execution time of \emph{Greedy} is 3 orders of magnitude slower than its LP version.
%The results demonstrate the gains when using \emph{ALGO-Main} within a reasonable execution time; however, \textit{Greedy} is much faster, and \textit{LP-MOSEK} cannot achieve the high performance of \emph{ALGO-Main} while is much slower than \textit{Greedy}. 
%Table~\ref{table:myopic-mosek-comparison} further highlights that it is preferable to solve \eq{eq:single-step-LP} with \textit{Greedy} than simply plugging it in a generic solver.\pavlos{I also think that Table~\ref{table:myopic-mosek-comparison} is a bit redundant and could be omitted to save space. Also, IMPORTANT, the results in the two tables for K=1000 are inconsistent}

%We present two tables, one showing the tradeoff of greedy myopic, LP-MOSEK myopic and ADMM in terms of optimizing Opt~\ref{problem:basis} and execution time for a synthetic scenario ($C/K = 0.8\%, N=2, Q = 90\%, s = 0.5~\text{(zipf exponent)}$) for a library of 1K contents, and a second one capturing only the execution time of LP-myopic and Greedy Myopic. Table~\ref{table:lp-myopic-lp-greedy-admm-comparison}, shows the immense improvement we get in terms performance with a reasonable execution time when using ADMM, while Table~\ref{table:myopic-mosek-comparison} shows it is preferable to solve GCFR with the method of Lemma~\ref{greedy-method} than simply plugging it in a generic solver.

\vspace{5pt}
\begin{table}[H]
\centering
\caption{LP-Myopic vs Greedy-Myopic vs ALGO-Main}\label{table:lp-myopic-lp-greedy-admm-comparison}
\begin{small}
\begin{tabular}{l|l|l|l}
%\hline
{}						&{LP-MOSEK} &{Greedy} &{ALGO-Main}\\
\hline \hline
{Hit rate (\%)}			&{11.13} &{11.17} &{21.51}\\
\hline
{Execution time (sec)}			&{140.58} &{0.09} &{553.19}\\
\hline

\end{tabular}
\end{small}
\end{table}


%\begin{table} 
%\centering 
%\caption{Execution times (sec) vs Library size \theo{a bit redundant I think}}\label{table:myopic-mosek-comparison}
%\begin{small}
%\begin{tabular}{l|l|l|l}
%\hline
%{}						&{200} &{1000} &{2000}\\
%\hline \hline
%{LP-mosek}				&{1.1668} &{130.039} &{1137.2}\\
%\hline
%{MyopicAlgo}			&{0.0556} &{0.1418} &{0.3987}\\
%\hline

%\end{tabular}
%\end{small}
%\end{table}


\subsection{Hybrid Algorithm}
\label{sec:hybrid}


%Commercial solvers are used to optimally solve convex problems, like the ones we defined as our subproblems of Section \secref{sec:optim_methods}. Although able to do so, they are typically implemented based on variants of interior-point method, a class of numerical algorithms which is really accurate but is unfortunately also slow. 

As shown above, \textit{Greedy} offers a tradeoff: fast vs. suboptimal cache-friendly recommendations. Here, we aim to achieve the best of both worlds, by combining \emph{ALGO-Main} (performance) and \textit{Greedy} (speed).

%As we will show in~\secref{sec:sims}, the proposed method outperforms commercial solvers in terms of execution time, managing to return equally accurate solutions. Typically, our scheme requires less than 30 minutes to converge in a library of $\simeq 1000$ contents (1M variables). Nonetheless, for a for realistic catalogs might lead to an order of magnitude more variables, and for such scenarios our ADMM-based method might be slow.

%\theo{Typically, the execution time of \ref{alg:ADMM} for a library of 1000 contents (i.e 1M optimization variables) is between 15-20 minutes. In a practical scenario, a recommendation system has to be in control of a library of size 2-5K contents. this needs to go earlier with the table Akis pointed}
%It is evident that when we need to deal with order of 10M variables it becomes a necessity to scale up the ADMM-based algorithm so it can catch up with realistic scenarios.

%Online content popularities are known to be heavy tailed distributed \cite{adamic2002zipf}. Based on this, we recommend a hybrid strategy that combines the ADMM-based method and the Myopic algorithm. As an example, assume a catalog of 2K contents with really skewed a priori distribution ($\mathbf{p_0}$). Then covering $\simeq 90\%$ of the popularities would be possible if we consider an order of magnitude smaller catalog with the most popular items. \pavlos{the 90\% seems (and is) totally arbitrary; could be supported with some data. If you agree, let me know and I can check if it's possible to get any numbers out of our dataset. BUT, in any case I think we should have this percentage as a input parameter in the algorithm.}

Our main idea is to apply the exact, optimal \emph{ALGO-Main} only to a small but important part of the recommendation matrix $\mathbf{R}$, and select the remaining recommendation variables with the fast \textit{Greedy} algorithm. The fact that content popularity distributions are skewed, motivates us to focus on the part of the matrix $\mathbf{R}$ corresponding to the most popular contents. This gives rise to \emph{ALGO-Hybrid} (Algorithm~\ref{alg:hybrid}). The following lemma gives some analytical insight into its workings.
% \begin{enumerate}[leftmargin=*]
% \item  Sort the rows and columns of matrix $\mathbf{U}$ in decreasing order of $\mathbf{p}_0$ (i.e., row 1 and column 1 correspond to content $i=\arg\max_{j\in\mathcal{K}}p_{j}$). 

% \item Start removing rows and columns, one-by-one, starting from the less popular content (row $K$ / column $K$).

% \item Every time a row and column is removed, check the remaining matrix $\mathbf{R^{\prime}}$ to ensure that the required quality constraint of Eq.(\ref{quality-con}) can still be satisfied.
% \item Stop either when step 3 fails or when the sum of popularities of the remaining elements drops below a value $P_{min}$. We are now left with a shrunk matrix $\mathbf{R^{\prime}}$ of size $K^{\prime}$.
% \item Apply Algorithm~\ref{alg:ADMM} to the $K^{\prime} \times K^{\prime}$ matrix $\mathbf{R^{\prime}}$. Apply \textit{Greedy} to the $K-K^{\prime}$ least popular contents (i.e., to $K-K^{\prime}$ rows and $K$ columns or the original matrix).% $K^{\prime} \times K$ submatrix, corresponding to $K-K^{\prime}$ least popular rows or the original matrix.
% \end{enumerate}

%\begin{definition}
%\emph{(Step 1)} Arrange the rows and column of matrix $\mathbf{U}$ in decreasing order of $\mathbf{p}$ (i.e., row 1 and column 1 correspond to the max $p_0^{i}$). \emph{(Step 2)} Start removing rows and columns, one-by-one, starting from row and column $K$. \emph{(Step 2b)} Every time a row and column is removed, check the remaining matrix $\mathbf{R^{\prime}}$ to ensure that the required quality constraint of Eq.(\ref{quality-con}) can still be satisfied. \emph{(Step 3)} Stop either when step 2b fails or when the sum of popularities of the remaining elements drops below a value $P_{min}$. Let us assume that the resulting shrunk matrix $\mathbf{R^{\prime}}$ is left with $K^{\prime}$ rows and lines. \emph{(Step 4)} Apply Algorithm~\ref{alg:ADMM} to $K^{\prime} \times K^{\prime}$ matrix $\mathbf{R^{\prime}}$. Apply Fast Greedy to the $K^{\prime} \times K$  submatrix, corresponding to $K-K^{\prime}$ least popular rows or the original matrix.
%\end{definition}
%\pavlos{it can be presented much simpler: it's just a hypergeometric distribution. no?}
\begin{lemma} \label{lemma:related-k-prime}
Assume that (i) each row of matrix $\mathbf{U}$ has exactly $L$ related items (i.e., entries equal to $1$), uniformly chosen among all other $K-1$ contents, and (ii) we randomly pick $K^{\prime} < K$ columns of $\mathbf{U}$. Then, for a randomly chosen row, the probability of the event that at least $N$ of the $L$ related items are left in the $K^{\prime}$ selected columns, is given by%Then, the probability there are at least $N$ of the $L$ related items left (for any row of $\mathbf{U}$) in the $K^{'}$ selected columns for the randomly chosen row of, is given by
%
%Assume that each row of matrix $\mathbf{U}$ has exactly $L$ related items (i.e., entries equal to $1$), uniformly chosen among all other $K-1$ contents. Assume further that we pick $K^{'} < K$ columns for each item. Then, the probability there are at least $N$ of the $L$ related items left (for any row of $\mathbf{U}$) in the selected columns for the randomly chosen row of, is given by
%\begin{small}
\begin{align} \label{pshrink-def}
P_{\text{shrink}} = \bigg(\sum_{n=N}^{L} \binom{L}{n} \Big(\frac{K^{\prime}}{K}\Big)^{n} \Big(1-\frac{K^{\prime}}{K}\Big)^{L-n}\bigg)^{K^{\prime}}
\end{align}



\begin{proof}
Assume a randomly picked row of $\mathbf{U}$ as a vector of $K$ entries. Given that an entry is nonzero uniformly (i.e. with prob. $\frac{1}{K}$), the probability that a specific subset of $K^{\prime}$ entries has a nonzero entry is equal to $K^{\prime}/K$. Then the probability that this subset has \emph{exactly} $n$ nonzero entries out of the possible $L$ existing ones follows a binomial distribution, we call this $p = \binom{L}{n} (\frac{K^{\prime}}{K})^{n} (1-\frac{K^{\prime}}{K})^{L-n}$. 
Nonetheless, we are interested for the event of having  \emph{at least} $n$ successes, which is why we sum from $n$ until $L$ in Eq.(\ref{pshrink-def}). Finally, we are interested in the event of having this event happening in $K^{\prime}$ different rows, but the probability of the event we calculated is the same for every row and is also \emph{independent of the row}, which explains the exponent ($K^{\prime}$) in Eq.(\ref{pshrink-def}).
\end{proof}
% Furthermore, the probability that the above is satisfied in all $K^{\prime}$ rows is $P_{\text{shrink}} = p^{K^{\}}$, as the events are independent.
%\end{small}
\end{lemma}



The above lemma can be used to estimate how small a $K^{\prime}$ value we can expect in practice. %Keep in mind that we are interested in having $N$ related items in all $K^{\prime}$ rows as well. 
% \theo{Note that $P_{shrink}$ is a function of many variables, namely of the form $f(N,L,K,K^{'})$, and one can study its behavior as a function of some of its variables simply by fixing some others.}
As an example, we demonstrate a synthetic case of two libraries with $K$=4000 contents and varying average densities ($L/K$) of related contents. In Fig.\ref{fig:binomial-cdf}, we present $P_{\text{shrink}}$ versus the value $K^{\prime}/K$. 
As we can see, $P_{\text{shrink}}$ becomes almost 1 (y-axis) for $K^{\prime}/K \approx 0.25$ (x-axis), which indicates that \emph{ALGO-Main} would need to be applied only to 1/4 of the initial content catalog $K$. 

Lemma~\ref{lemma:related-k-prime} makes a simplistic assumption for the structure of matrix $\mathbf{U}$. For example, studies have found~\cite{sermpezis-sch-globecom} %(and our data traces also confirm)
that related items tend to be chosen among the more popular ones. This implies that Lemma~\ref{lemma:related-k-prime} provides a pessimistic value of $P_{\text{shrink}}$; in practice smaller values $K^{\prime}$ are feasible. %In the next section, we compare the performance of this Hybrid algorithm to the original.
\vspace{5pt}
\begin{algorithm}[h]
\begin{small}
\begin{algorithmic} [1]
\caption{ALGO-Hybrid}\label{alg:hybrid}
\State Sort the rows and columns of matrix $\mathbf{U}$ in decreasing order of $\mathbf{p}_0$ (i.e., row / column 1 correspond to content $i=\arg\max_{j\in\mathcal{K}}p_{j}$). 

\State Start removing rows and columns, one-by-one, starting from the less popular content (row $K$ / column $K$).

\State Every time a row and column is removed, check the remaining matrix $\mathbf{R^{\prime}}$ to ensure that the required quality constraint of Eq.(\ref{quality-con}) can still be satisfied.

\State Stop either when step 3 fails or when the sum of popularities of the remaining elements drops below a value $P_{min}$. We are now left with a shrunk matrix $\mathbf{R^{\prime}}$ of size $K^{\prime}$.

\State Apply \emph{ALGO-Main} to the $K^{\prime} \times K^{\prime}$ matrix $\mathbf{R^{\prime}}$. Apply \textit{Greedy} to the $K-K^{\prime}$ least popular contents (i.e., to $K-K^{\prime}$ rows and $K$ columns or the original matrix).
\end{algorithmic}
\end{small}
\end{algorithm}



%For example..." point to the figure explaining what you're plotting and comment on the result, STRESSING that indeed K' can be small enough. Then say

%The main idea is to pick the ``important'' part of $\mathbf{U}$ that corresponds to the most popular set of items (covering around 90\% of total popularity). We could then apply at this part the ADMM-based algorithm so the performance of the method is not heavily compromised. For the remaining catalog, we opt to apply the \textit{FM} in order to gain valuable execution time for the whole algorithm. A reasonable approach to achieve the shrinking of the catalog, would be to focus on the part of $\mathbf{U}$ corresponding to the very popular items, and start picking their rows and their respective columns. However, we should be careful as removing columns means removing related contents, and the quality constraint Eq.(\ref{quality-con}) might not be able to be satisfied, no matter what we recommend. Hence, we need an organized method that will ensure that the sub-matrix chosen can still give feasible solution. To achieve this we start removing rows and columns starting from the least popular content and check if the quality constraint (i.e entries of $\mathbf{U}$ suffice for the required $q$). The method which returns this new $\mathbf{U}$ is described as follows.

%\begin{algorithm}[H]
%\begin{algorithmic} [1]
%\caption{$\mathbf{U}$ shrinking}\label{alg:hybrid}
%\Statex {Input: $N,~q,~\mathbf{U}$} 
%\Statex {Output: $\mathbf{U}^{\prime}$} 

%\State {Order popularities}
%\State {$i \gets K$}
%\State {$p \gets 1$}
%\State {$t \gets \sum_{j \in \mathcal{R}_{i}} u_{ij}$}
%\Repeat 
%\State {$\mathbf{U}_{i,\cdot},~\mathbf{U}_{\cdot,i} \gets []$}
%\State {$t \gets \sum_{j = 0}^{i} u_{ij}$}
%\State {$p \gets p - p_{0}^{i}$}
%\State {$i \gets i-1$}
%\State {$v\gets (p\le 0.9) \lor (t\le qN)$}
%\Until \{$(p \le 0.9) \lor (t < qN)$ is False\}
%\State {return $\mathbf{U}^{\prime} \gets \mathbf{U}$}
%\end{algorithmic}
%\end{algorithm}

%Before we present the idea of the algorithm, we need to analyze two key problem parameters and establish some mild conditions under which the hybrid strategy may be applicable.

%\textbf{The role of $N$ and $q$.}
%To facilitate our analysis, assume that $u_{ij}$ is binary. In doing so, the quality constraint \ref{quality-con} can be reduced in $\sum_{j \in \mathcal{R}_{i}} y_{ij} \ge q,~\forall ~i \in \mathcal{K}$, where $\mathcal{R}_i$ is the set of related elements for content $i$. 
%Now given that $y_{ij}$ is imposed on~\ref{box-con}, to achieve the extreme case $q = 100\%$ and guarantee feasibility of the problem, we need the condition $R_{i} \geq N~\forall~i \in \mathcal{K}$ to hold.

%Further assume now that the contents are ordered based on decreasing popularity. Our goal is to reduce the size of $\mathbf{U}$ 
%We propose a simple algorithm that starts from the least popular item and removes rows and columns from $U$ until we cannot a find a row of $U$ with less than $N$ contents, thus leaving us with a square matrix $U_{1} \in \mathcal{R}^{k_{1} \times k_{1}}$. We call this new set of contents $\mathcal{K}_{1}$.


%a) the algorithm description is terrible. basically it's impossible to understand what you propose, and why you need to probabilistic analysis (that follows)

%b) in the previous section, we described our algorithms clearly and wrote the code. why did we drop this style in this section?? you should write the algorithm explicitly. and in trying to write it correctly, you will also see how you should explain it.

%but overall the idea is simple:
%1) we want to pick a (hopefully much) smaller part of the matrix Y, but still a square one, to apply our ADMM algorithm on. this should be the "important" part of the matrix, to ensure that the overall performance is not heavily compromised.
%2) for the rest of the matrix we'll run sth much simpler (namely fast myopic) to gain valuable execution time.
%3) A reasonable thing to do to achieve (1) is to focus on popular items, and pick the rows corresponding to the most popular items only, together with the respective columns.
%4) However, we must be careful as removing columns means removing related contents, and the quality constraint (eq...) might not be able to be satisfied, *no matter what we recommend*.
%5) Hence, we need an "organized" method that will ensure that the sub-matrix chosen can still give feasible solution. to achieve this we start removing rows starting from unpopular contents and check the quality constraint of....until....


%\textbf{Modeling the process.} The above algorithm returns a $\mathbf{U}^{\prime}$ which can give a feasible solution and guarantees that its remaining $k^{\prime}$ contents cover at least a 90\% of $\mathbf{p}$. However, we have not yet made any claims on the new size $k^{\prime}$. To address this, we have to look back at $\mathbf{U}$ and take into consideration the average number of related contents $\mathbf{E}[U_i]$. Essentially we pose the question \textit{"What is the average $U_{i}$ which guarantees with high probability that the resulting $U^{\prime}$ will have at least $N$ related contents in all its $k^{\prime}$ rows"}.

%\theo{@Akis, we might get shot for saying that the relations are uniformly distributed, which eases our approach but probably is not that realistic. Data has structure, and I think here we make a dangerous claim by assuming total randomness, if the paper reaches guys like Pavlos we're scr@wed. On the bright side, the structure would probably help our method, as I believe the probability riana is related to kanye west is a loooot more probable than riana to be related with fishing tips video. Dont kill me, but I think that if we change the analyis and make this $p=k^{\prime}/k$ somehow related to $\mathbf{p}$ we have two wins. First we assume normal things, and secondly as riana is more likely to be related to beyonce, the size k prime is more likely to be even smaller if you think about it.}


%A random row of $U$ has on average $\mathbf{E}[U_i]=M$ related contents and we choose a subset of this row of size $k^{\prime}$. Assuming that the 1's are uniformly distributed in the $k$ positions of the row, the probability to find these $M$ 1's in the $k^{\prime}$ size subset will simply be $p=k^{\prime}/k$. If we pick a row of $\mathbf{U}$, the probability to land \textit{at least} $N$ 1's in the subset $k^{\prime}$ when there exist $M$ 1's in the $k$ positions, could be seen as an analogy to the fundamental balls and bins problem. Therefore, for every $i$-th row, it could be computed as 

%\begin{small}
%\begin{align}
%p_{i} = P(U_i \ge N) = \sum_{n=N}^{M} \binom{M}{n} p^{n} (1-p)^{M-n}
%\end{align}
%\end{small}
%The per row statistics are assumed to be independent, so the probability that all rows have at least $N$ 1's is simply the product of $p_{i}$ $k^{\prime}$ times, i.e $p_{i}^{k^{\prime}}$. \todo{here we should include the comment about the structure of the dataset, and stress that this simple analysis serves somehow as a a worst case}. As an example we demonstrate a synthetic case of a library with 4K contents and different average densities (in \% terms) of related contents. In Fig.\ref{fig:binomial-cdf}, we visualize the probability the sub-matrix (of size $k^{\prime}$) to have at least $N$ ace entries for different values $\mathbf{E}[U_i]$, versus the increasing normalized $k^{\prime}$.

\begin{figure}[]
\centering
\subfigure[last.fm,~($s = 0.6$,~$q=80\%$,~$C/K=1.32\%$)]{\includegraphics[width=0.4\columnwidth]{lastfm_admm_convergence_v3}\label{fig:last-fm-convergence}}
%\subfigure[Youtube~\cite{youtube-related-videos-dataset},~$N = 2,~s = 0.6,~Q=80\%,~C/K=1.32\%$]{\includegraphics[width=0.4\columnwidth]{Youtube_admm_convergence}\label{fig:last-fm-convergence}}
\hspace{0.08\columnwidth}
\subfigure[$P_{\text{shrink}}$ vs $K^{\prime}/K$]{\includegraphics[width=0.4\columnwidth]{binomial_utility_cdf_v2}\label{fig:binomial-cdf}}
\vspace{-2.5mm}
\caption{ALGO-Main Convergence \& $P_{\text{shrink}}$.}
\end{figure}

%\pavlos{in ``(b)'': (i) what is the $R_{i}$ in the legend. Use $L/K$. (ii) the values of L/K are similar; use either other values, e.g., [0.001, 0.01, 0.1], or (for min effort) only one curve. (iii) what is k1 in the xlabel? (iv) verify that the values of L/K are percentages? they seem too small}

%The above analysis serves as an assurance mechanism that indicates in which cases our strategy is applicable. 

%The matrix $\mathbf{R}_{1} \in \mathbb{R}^{k_{1} \times k_{1}}$ depicts the recommendation probabilities for the most popular contents and is based on the ADMM policy while $\mathbf{R}_{2} \in \mathbb{R}^{(k-k_{1}) \times k_{2}}$ is calculated using the \textit{FM} method. Having said that the square matrix of size $K$ $\mathbf{R}$ will have the form $\mathbf{R}=[\mathbf{R}_1 \quad \mathbf{0}_{k_1 \times (k-k_{1})}~ \mathbf{;} ~\mathbf{R}_2]$.

%Having said that, and if we call $Y_{1}$, the recommender for the most popular part, $Y_{2}$ the respective for the less important subset of contents, the overall square matrix of size $K$ will be $Y$ will have the form $Y=[Y_1 \mathbf{0}_{k_1 \times (k-k_{1})} ; Y_2]$.

%\[
%\begin{bmatrix}
%	M_1 & | & \mathbf{0} \\
 %   \\
  %  \hline \\
   % &M_2
%\end{bmatrix}
%\]
%\[
%\left[ 
%\begin{array}{lcr}
%		M_{1}  & | & \mathbf{0}_{k_1 \times (k-k_{1})}  \\ \hline
 %       & & \\
  %      & \qquad M_{2} & \\
   %   &  &
%\end{array}\right]
%\]

%-Zipfian popularity of online contents gives us a hint on how to reduce our schemes complexity by grouping the 90$\%$ of the total pmf.

%-Give the necessary condition that need to hold for the utility matrix. Use the analogy of balls and bins to show with the cdf how many related we need on average in order to reduce the size of the problem (significantly).

%-Visually present the solution we have in mind by giving out the large matrix and explain how the method works on its respective blocks.


==> hybrid_method.tex <==
%Commercial solvers are used to optimally solve convex problems, like the ones we defined as our subproblems of Section \secref{sec:optim_methods}. Although able to do so, they are typically implemented based on variants of interior-point method, a class of numerical algorithms which is really accurate but is unfortunately also slow. 


As we just saw, the fast greedy algorithm offers a tradeoff, fast but suboptimal cache-friendly recommendations. In this last section, we show that one can often have the best of both worlds, by combining the two algorithms presented

%As we will show in~\secref{sec:sims}, the proposed method outperforms commercial solvers in terms of execution time, managing to return equally accurate solutions. Typically, our scheme requires less than 30 minutes to converge in a library of $\simeq 1000$ contents (1M variables). Nonetheless, for a for realistic catalogs might lead to an order of magnitude more variables, and for such scenarios our ADMM-based method might be slow.

%\theo{Typically, the execution time of \ref{alg:ADMM} for a library of 1000 contents (i.e 1M optimization variables) is between 15-20 minutes. In a practical scenario, a recommendation system has to be in control of a library of size 2-5K contents. this needs to go earlier with the table Akis pointed}
%It is evident that when we need to deal with order of 10M variables it becomes a necessity to scale up the ADMM-based algorithm so it can catch up with realistic scenarios.

%Online content popularities are known to be heavy tailed distributed \cite{adamic2002zipf}. Based on this, we recommend a hybrid strategy that combines the ADMM-based method and the Myopic algorithm. As an example, assume a catalog of 2K contents with really skewed a priori distribution ($\mathbf{p_0}$). Then covering $\simeq 90\%$ of the popularities would be possible if we consider an order of magnitude smaller catalog with the most popular items. \pavlos{the 90\% seems (and is) totally arbitrary; could be supported with some data. If you agree, let me know and I can check if it's possible to get any numbers out of our dataset. BUT, in any case I think we should have this percentage as a input parameter in the algorithm.}

Our main idea is to apply the exact, optimal algorithm Algorithm~\ref{alg:ADMM} only to a small part of the recommendation matrix $\mathbf{R}$. Then, for the rest of the recommendation variables, to pick them greedily (albeit suboptimally) with the Fast Greedy method. Given that content popularity distributions tend to be skewed~\cite{adamic2002zipf}, it is reasonable to focus on the part of the matrix corresponding to the most popular contents. Our Hybrid algorithm works as follows:

\begin{enumerate}[leftmargin=*]
\item  Arrange the rows and column of matrix $\mathbf{U}$ in decreasing order of $\mathbf{p}_0$ (i.e., row 1 and column 1 correspond to the max $p_0^{i}$). 

\item Remove rows and columns, one-by-one, starting from content $K$.

\item Every time a row and column is removed, check the remaining matrix $\mathbf{R^{\prime}}$ to ensure that the required quality constraint of Eq.(\ref{quality-con}) can still be satisfied.
\theo{when $q=f(q_{max})$ this can always be satisfied}

\item Stop either when step 3 fails or when the sum of popularities of the remaining elements drops below a value $P_{min}$. We are now left with a shrunk matrix $\mathbf{R^{\prime}}$ of size $K^{\prime}$.

\item Apply Algorithm~\ref{alg:ADMM} to $K^{\prime} \times K^{\prime}$ matrix $\mathbf{R^{\prime}}$. Apply Fast Greedy to the $K^{\prime} \times K$  submatrix, corresponding to $K-K^{\prime}$ least popular rows or the original matrix.
\end{enumerate}


%\begin{definition}
%\emph{(Step 1)} Arrange the rows and column of matrix $\mathbf{U}$ in decreasing order of $\mathbf{p}$ (i.e., row 1 and column 1 correspond to the max $p_0^{i}$). \emph{(Step 2)} Start removing rows and columns, one-by-one, starting from row and column $K$. \emph{(Step 2b)} Every time a row and column is removed, check the remaining matrix $\mathbf{R^{\prime}}$ to ensure that the required quality constraint of Eq.(\ref{quality-con}) can still be satisfied. \emph{(Step 3)} Stop either when step 2b fails or when the sum of popularities of the remaining elements drops below a value $P_{min}$. Let us assume that the resulting shrunk matrix $\mathbf{R^{\prime}}$ is left with $K^{\prime}$ rows and lines. \emph{(Step 4)} Apply Algorithm~\ref{alg:ADMM} to $K^{\prime} \times K^{\prime}$ matrix $\mathbf{R^{\prime}}$. Apply Fast Greedy to the $K^{\prime} \times K$  submatrix, corresponding to $K-K^{\prime}$ least popular rows or the original matrix.
%\end{definition}

%\pavlos{it can be presented much simpler: it's just a hypergeometric distribution. no?}

\begin{lemma} \label{lemma:related-k-prime}
Assume that each row of matrix $\mathbf{U}$ has exactly $U_i = L$ related items, uniformly chosen among all other ($K-1$) contents. Assume further that we pick $K^{'} < K$ columns for each item. Then, the probability there are at least $N$ of the $L$ related items left (for any row of $\mathbf{U}$) in the selected columns for the randomly chosen row of, is given by
\begin{small}
\begin{align}
p = f(\frac{K^{\prime}}{K}) = \sum_{n=N}^{L} \binom{L}{n} (\frac{K^{\prime}}{K})^{n} (1-\frac{K^{\prime}}{K})^{L-n}
\end{align}
\end{small}
\end{lemma}

The above lemma can be used to estimate how small a $K^{\prime}$ value we can hope for in practice. Keep in mind that we are interested in having $N$ related items in all $K^{\prime}$ rows as well. As an example we demonstrate a synthetic case of three libraries with 4K contents and different average densities (in $L/K$ \% terms) of related contents. In Fig.\ref{fig:binomial-cdf}, we present the probability the square sub-matrix (of size $K^{\prime}$) (computed as $p^{K^{\prime}}$) to have at least $N$ related items versus the increasing $K^{\prime}/K$. As we can see, when $K^{\prime}/K \approx 0.25$, means we are near-certain that we can pick a catalog of 1/4 of the initial size $K$ and which has the necessary entries to allow us to apply Algorithm~\ref{alg:ADMM}. Of course, the model of Lemma~\ref{lemma:related-k-prime} is quite simplistic, compared to the actual structure of matrix $\mathbf{U}$. For example, studies have found (and our data traces also confirm) that related items tend to be chosen among the more popular ones, everything else equal. This however can work in our favor, as the above result would in fact be pessimistic. We will compare the perfomance of this Hybrid scheme to the original in the next section.

%For example..." point to the figure explaining what you're plotting and comment on the result, STRESSING that indeed K' can be small enough. Then say

%The main idea is to pick the ``important'' part of $\mathbf{U}$ that corresponds to the most popular set of items (covering around 90\% of total popularity). We could then apply at this part the ADMM-based algorithm so the performance of the method is not heavily compromised. For the remaining catalog, we opt to apply the \textit{FM} in order to gain valuable execution time for the whole algorithm. A reasonable approach to achieve the shrinking of the catalog, would be to focus on the part of $\mathbf{U}$ corresponding to the very popular items, and start picking their rows and their respective columns. However, we should be careful as removing columns means removing related contents, and the quality constraint Eq.(\ref{quality-con}) might not be able to be satisfied, no matter what we recommend. Hence, we need an organized method that will ensure that the sub-matrix chosen can still give feasible solution. To achieve this we start removing rows and columns starting from the least popular content and check if the quality constraint (i.e entries of $\mathbf{U}$ suffice for the required $q$). The method which returns this new $\mathbf{U}$ is described as follows.

%\begin{algorithm}[H]
%\begin{algorithmic} [1]
%\caption{$\mathbf{U}$ shrinking}\label{alg:hybrid}
%\Statex {Input: $N,~q,~\mathbf{U}$} 
%\Statex {Output: $\mathbf{U}^{\prime}$} 

%\State {Order popularities}
%\State {$i \gets K$}
%\State {$p \gets 1$}
%\State {$t \gets \sum_{j \in \mathcal{R}_{i}} u_{ij}$}
%\Repeat 
%\State {$\mathbf{U}_{i,\cdot},~\mathbf{U}_{\cdot,i} \gets []$}
%\State {$t \gets \sum_{j = 0}^{i} u_{ij}$}
%\State {$p \gets p - p_{0}^{i}$}
%\State {$i \gets i-1$}
%\State {$v\gets (p\le 0.9) \lor (t\le qN)$}
%\Until \{$(p \le 0.9) \lor (t < qN)$ is False\}
%\State {return $\mathbf{U}^{\prime} \gets \mathbf{U}$}
%\end{algorithmic}
%\end{algorithm}

%Before we present the idea of the algorithm, we need to analyze two key problem parameters and establish some mild conditions under which the hybrid strategy may be applicable.

%\textbf{The role of $N$ and $q$.}
%To facilitate our analysis, assume that $u_{ij}$ is binary. In doing so, the quality constraint \ref{quality-con} can be reduced in $\sum_{j \in \mathcal{R}_{i}} y_{ij} \ge q,~\forall ~i \in \mathcal{K}$, where $\mathcal{R}_i$ is the set of related elements for content $i$. 
%Now given that $y_{ij}$ is imposed on~\ref{box-con}, to achieve the extreme case $q = 100\%$ and guarantee feasibility of the problem, we need the condition $R_{i} \geq N~\forall~i \in \mathcal{K}$ to hold.

%Further assume now that the contents are ordered based on decreasing popularity. Our goal is to reduce the size of $\mathbf{U}$ 
%We propose a simple algorithm that starts from the least popular item and removes rows and columns from $U$ until we cannot a find a row of $U$ with less than $N$ contents, thus leaving us with a square matrix $U_{1} \in \mathcal{R}^{k_{1} \times k_{1}}$. We call this new set of contents $\mathcal{K}_{1}$.


%a) the algorithm description is terrible. basically it's impossible to understand what you propose, and why you need to probabilistic analysis (that follows)

%b) in the previous section, we described our algorithms clearly and wrote the code. why did we drop this style in this section?? you should write the algorithm explicitly. and in trying to write it correctly, you will also see how you should explain it.

%but overall the idea is simple:
%1) we want to pick a (hopefully much) smaller part of the matrix Y, but still a square one, to apply our ADMM algorithm on. this should be the "important" part of the matrix, to ensure that the overall performance is not heavily compromised.
%2) for the rest of the matrix we'll run sth much simpler (namely fast myopic) to gain valuable execution time.
%3) A reasonable thing to do to achieve (1) is to focus on popular items, and pick the rows corresponding to the most popular items only, together with the respective columns.
%4) However, we must be careful as removing columns means removing related contents, and the quality constraint (eq...) might not be able to be satisfied, *no matter what we recommend*.
%5) Hence, we need an "organized" method that will ensure that the sub-matrix chosen can still give feasible solution. to achieve this we start removing rows starting from unpopular contents and check the quality constraint of....until....


%\textbf{Modeling the process.} The above algorithm returns a $\mathbf{U}^{\prime}$ which can give a feasible solution and guarantees that its remaining $k^{\prime}$ contents cover at least a 90\% of $\mathbf{p}$. However, we have not yet made any claims on the new size $k^{\prime}$. To address this, we have to look back at $\mathbf{U}$ and take into consideration the average number of related contents $\mathbf{E}[U_i]$. Essentially we pose the question \textit{"What is the average $U_{i}$ which guarantees with high probability that the resulting $U^{\prime}$ will have at least $N$ related contents in all its $k^{\prime}$ rows"}.

%\theo{@Akis, we might get shot for saying that the relations are uniformly distributed, which eases our approach but probably is not that realistic. Data has structure, and I think here we make a dangerous claim by assuming total randomness, if the paper reaches guys like Pavlos we're scr@wed. On the bright side, the structure would probably help our method, as I believe the probability riana is related to kanye west is a loooot more probable than riana to be related with fishing tips video. Dont kill me, but I think that if we change the analyis and make this $p=k^{\prime}/k$ somehow related to $\mathbf{p}$ we have two wins. First we assume normal things, and secondly as riana is more likely to be related to beyonce, the size k prime is more likely to be even smaller if you think about it.}


%A random row of $U$ has on average $\mathbf{E}[U_i]=M$ related contents and we choose a subset of this row of size $k^{\prime}$. Assuming that the 1's are uniformly distributed in the $k$ positions of the row, the probability to find these $M$ 1's in the $k^{\prime}$ size subset will simply be $p=k^{\prime}/k$. If we pick a row of $\mathbf{U}$, the probability to land \textit{at least} $N$ 1's in the subset $k^{\prime}$ when there exist $M$ 1's in the $k$ positions, could be seen as an analogy to the fundamental balls and bins problem. Therefore, for every $i$-th row, it could be computed as 

%\begin{small}
%\begin{align}
%p_{i} = P(U_i \ge N) = \sum_{n=N}^{M} \binom{M}{n} p^{n} (1-p)^{M-n}
%\end{align}
%\end{small}
%The per row statistics are assumed to be independent, so the probability that all rows have at least $N$ 1's is simply the product of $p_{i}$ $k^{\prime}$ times, i.e $p_{i}^{k^{\prime}}$. \todo{here we should include the comment about the structure of the dataset, and stress that this simple analysis serves somehow as a a worst case}. As an example we demonstrate a synthetic case of a library with 4K contents and different average densities (in \% terms) of related contents. In Fig.\ref{fig:binomial-cdf}, we visualize the probability the sub-matrix (of size $k^{\prime}$) to have at least $N$ ace entries for different values $\mathbf{E}[U_i]$, versus the increasing normalized $k^{\prime}$.

\begin{figure}[]
\centering
\subfigure[LastFM,~($s = 0.6$,~$Q=80\%$,~$C/K=1.32\%$)]{\includegraphics[width=0.4\columnwidth]{lastfm_admm_convergence}\label{fig:last-fm-convergence}}
%\subfigure[Youtube~\cite{youtube-related-videos-dataset},~$N = 2,~s = 0.6,~Q=80\%,~C/K=1.32\%$]{\includegraphics[width=0.4\columnwidth]{Youtube_admm_convergence}\label{fig:last-fm-convergence}}
\subfigure[$p^{K^{\prime}}$ vs $K^{\prime}/K$]{\includegraphics[width=0.4\columnwidth]{binomial_utility_cdf}\label{fig:binomial-cdf}}
\caption{ADMM conjecture \& Probability $p^{K^\prime}$.}
\end{figure}

%The above analysis serves as an assurance mechanism that indicates in which cases our strategy is applicable. 

%The matrix $\mathbf{R}_{1} \in \mathbb{R}^{k_{1} \times k_{1}}$ depicts the recommendation probabilities for the most popular contents and is based on the ADMM policy while $\mathbf{R}_{2} \in \mathbb{R}^{(k-k_{1}) \times k_{2}}$ is calculated using the \textit{FM} method. Having said that the square matrix of size $K$ $\mathbf{R}$ will have the form $\mathbf{R}=[\mathbf{R}_1 \quad \mathbf{0}_{k_1 \times (k-k_{1})}~ \mathbf{;} ~\mathbf{R}_2]$.

%Having said that, and if we call $Y_{1}$, the recommender for the most popular part, $Y_{2}$ the respective for the less important subset of contents, the overall square matrix of size $K$ will be $Y$ will have the form $Y=[Y_1 \mathbf{0}_{k_1 \times (k-k_{1})} ; Y_2]$.

%\[
%\begin{bmatrix}
%	M_1 & | & \mathbf{0} \\
 %   \\
  %  \hline \\
   % &M_2
%\end{bmatrix}
%\]
%\[
%\left[ 
%\begin{array}{lcr}
%		M_{1}  & | & \mathbf{0}_{k_1 \times (k-k_{1})}  \\ \hline
 %       & & \\
  %      & \qquad M_{2} & \\
   %   &  &
%\end{array}\right]
%\]

%-Zipfian popularity of online contents gives us a hint on how to reduce our schemes complexity by grouping the 90$\%$ of the total pmf.

%-Give the necessary condition that need to hold for the utility matrix. Use the analogy of balls and bins to show with the cdf how many related we need on average in order to reduce the size of the problem (significantly).

%-Visually present the solution we have in mind by giving out the large matrix and explain how the method works on its respective blocks.


==> introduction_old.tex <==
At the dawn of the era of 5G, we witness dramatic changes in \textit{network architecture} and \textit{user traffic demand}, two main elements that shape the ecosystem of modern and future mobile networks. 
%
New architectures for cellular networks, comprising densification of the access network (small-cells, SCs) and integration of computing and caching capabilities in base stations (mobile edge caching \& computing, MEC), have been proposed~\cite{bastug2014living}, to cope with the recent boom in traffic demand~\cite{networking2016forecast} and the envisioned increase in devices/traffic density in the near future ($\times10k$ more traffic and $\times10-100$ more devices~\cite{5GnumbersWashingtonPost}).
%
At the same time, the higher data rates offered by mobile operators, lead to changes in the consuming habits of users as well. Users nowadays consume more video and music traffic through their mobile devices (video will be $82\%$ of the total traffic by 2021~\cite{networking2016forecast}). 
%\rem{The special characteristics of this type of traffic, i.e., high bitrate and low latency, stretch further the quality requirements that mobile networks need to satisfy.}

%Mobile operators have experienced the last years an increase in the number of users and their traffic demand~\cite{networking2016forecast}, and both are expected to further increase in the near future ($\times10k$ more traffic and $\times10-100$ more devices~\cite{5GnumbersWashingtonPost}). To cope with the increasing density of devices/traffic, architectures comprising more base stations (small-cells, SCs), with smaller range and densely deployed, have been proposed~\cite{bastug2014living}. Moreover, introducing computing and caching capabilities in base stations (mobile edge caching/computing, MEC) can further help towards keeping traffic local, and thus offloading the backhaul, which can get congested at peak hours.

%The technological advances in mobile networks enable higher data rates, and this results in changes in the consuming habits of users as well. Users consume more and more video or music traffic through their mobile devices (video traffic will be 82\% of the total traffic by 2021~\cite{networking2016forecast}). The special characteristics of this type of traffic, i.e., high data rates and low latency, stretch the quality requirements that mobile networks need to satisfy.

%At a first sight, the advances in network architecture seem to be well-adapted to traffic demand. 
%\cite{breslau1999,adamic2002zipf}
Video (and music) traffic is highly skewed~\cite{youtube-traffic-from-edge,top-video-cellular,pptv-mobile-vod}, with a relatively small number of popular videos creating a large part of the demand. This skewness favors caching efficiency, and has made Content Distribution Networks (CDNs) a major component of today's wired Internet. Nevertheless, these ideas are not immediately applicable to future wireless networks. Even putting aside the interference-prone nature of the wireless channel, several factors limit the gains from mobile edge caching, in practice: (i) The size of content catalogues (even of only the most popular contents) is typically much larger than the storage capacity of a small base station. As a result, a large number of requests will always have to be redirected through the backhaul no matter what caching policy is used~\cite{Paschos-infocom2016, ElayoubiRoberts15}. (ii) The smaller coverage area of SCs implies frequent changes in the set of associated users in a SC, and this introduces larger variation in content request patterns. Thus, it becomes more difficult for a caching algorithm to accurately predict the ``local content popularity''~\cite{Paschos-infocom2016}. (iii) Viral videos routinely receive hundreds of thousands of views within a few hours after their upload~\cite{wikipedia-viral-videos} (and usually fade in equally fast). To accommodate for such trending videos, frequent updates of cached content is needed, which imposes a heavy load for the backhaul.
%However, there is a number of network and traffic characteristics that limit the gains from edge caching. Namely: (i) The size of content catalogues (even of only the most popular contents) is typically orders of magnitude larger than the caching capacity base stations. \rem{For example, ... [add sth similar to the discussion we have in the femto-caching paper]}. As a result, a large number of requests will always have to be redirected through the backhaul no matter what caching policy is used. (ii) The small coverage area of SCs (due to the densification of the network, and lower ranges) implies frequent changes in the set of associated users in a SC. Since users preferences vary, frequent changes of associated user introduces larger variation in content request patterns (local popularity). Thus, it becomes more difficult for caching algorithm to accurately predict the ``local content popularity''~\cite{Paschos-infocom2016}. (iii) Video popularity is highly time-varying. For example, a new VEVO video routinely receives 100s of thousands of views within a few hours after its upload. To accommodate for such trending videos that have the tendency to fade in users' requests intensity (as new ones get regularly uploaded), caching policies would require frequent update of caches, which still might be a heavy burden for backhaul.

A large number of \textit{cooperative caching} policies have been recently proposed aiming to improve wireless caching efficiency, by exploiting coverage overlaps of small-cells~\cite{femto,poularakis2014toc}, coded transmissions~\cite{Ali2014}, caching on user equipment~\cite{Hui-offloading,sermpezis2014,Pavlos-Offload2016} and vehicles~\cite{Whitbeck-offloading,vigneri2016}, and others~\cite{collaborative-multi-bitrate-caching}. While these policies do offer considerable benefits \textit{in theory}, and under certain conditions some practical gains as well, they also face the above obstacles (as well as some additional ones, e.g., subpacketization complexity~\cite{shanmugam2016finite}, limited resources in the case of device-side caching, etc.) 

The above discussion suggests that caching policy alone is limited in the amount of performance gain it can bring at a small edge cache. Increasing cache capacity (to improve hit rates) or backhaul capacity (to allow for more frequent updates) seem like the only way to cope with this problem, but these are ``hardware'' solutions involving significant CAPEX/OPEX costs, when considering the very large number of small base stations envisioned in future heterogeneous and ultra-dense networks. The following question then arises: 
\textit{Are there any practical ``software-based'' solutions that can improve caching efficiency, at a low cost?}
%The above characteristic imply that improving the gains of caching through improvement of caching policies (replacement/eviction algorithms) might be limited. Considerable gains could seem possible through (a) increase of caching capacity, or (b) more frequent update of cached content (which put extra load on backhaul, or fronthaul in some architectures~\rem{[cite]}). However, these approaches come with a need for ``hardware'' changes, i.e., upgrade of equipment (caches or backhaul, respectively), which is costly and might not be always feasible. Hence, a question that arises is: \textit{Are there cheap, practical, ``software-based'' solutions that can improve caching efficiency?}

Our answer to this question follows from two key observations: (i) the performance of a caching algorithm is dependent on user request patterns; (ii) user requests are increasingly driven by recommendation algorithms~\cite{cheng2009nettube,gupta2017modeling,RecImpact-IMC10}. For example, Netflix reports that around 80\% of its video views are through recommendations~\cite{gomez2016netflix}, while the corresponding percentage for YouTube's related video is 50\%~\cite{RecImpact-IMC10}. Our proposal is therefore to not try to further improve what is stored at each cache, but rather \textit{to better exploit the already cached content} by taking advantage of the recommendation algorithms, integrated in many of the content services that dominate the traffic consumption (e.g., YouTube, Netflix, Spotify). For instance, upon peak hours, when the backhaul is congested, a recommendation system could put higher preference on recommending content pre-cached in the vicinity of a user (e.g., at the base station with which she is associated, or to a nearby cache). 
%Several recent measurement studies~\cite{cheng2009nettube,gupta2017modeling,RecImpact-IMC10} have revealed that recommendation systems possess a vital role in shaping traffic demand. 

However, recommendations cannot be arbitrarily manipulated in practice. The recommendation system still needs to accomplish its primary goal, i.e., recommend to users contents of their interest. Hence, the goal of this paper is to \textit{leverage the recommendation system to increase the caching efficiency, while at the same time ensuring high quality recommendations}. Note also that, recommending a content that is almost as interesting to the user but locally cached might not just be ``acceptable to the user, better for the network'', but even \textit{beneficial to both the user and the network}, if that content can be streamed for example at better quality (since congested links are avoided). 

The idea of improving edge caching by taking into account recommendations has been recently proposed~\cite{sermpezis-sch-globecom,sch-chants-2016,chatzieleftheriou2017caching,liu2018learning}, by optimizing caching policies based on~\cite{sermpezis-sch-globecom,sch-chants-2016} or jointly with recommendation systems~\cite{chatzieleftheriou2017caching,liu2018learning}. These solutions require control over the caching policy (e.g., if content and network provider are the same entities or collaborate), which might not be feasible for every scenario. What is more, these works assume simple models of content access, such as the Independent Reference Model (IRM), where consecutive requests by a user are independent.
%and (b) focus only on the current request of a user, neglecting thus the long term behavior of users, who usually consume sequentially many contents.
In this paper, we go beyond the state of the art, by making the following contributions:

\pavlos{Some ideas (informally written) about the contribution we can state for this paper:
\begin{itemize}
\item We model the recommendation-driven user content access. The model allows us to formulate more accurately the problem, compared to existing models that assume single requests~\cite{merkouris, sch} or make long term approximations for sequential requests~\cite{wowmom}.
\item We propose efficient algorithms to solve the problem. We go beyond previous works, by (i) analytically investigating the hardness of the problem, and --based on this analysis-- (ii) designing algorithms with low complexity (for a hard problem) that can be applied in practice.
\end{itemize}
}


\begin{itemize}[leftmargin=*]
\item To our best knowledge, we propose the first model for recommendation-driven sequential user requests%
%we propose the first Markov chain based model for recommendation-driven user requests in this context
, that better fits real users behavior in a number of popular applications (e.g. YouTube, Vimeo, personalized radio). We then formulate the problem of maximizing the impact of recommendations on cache performance, while maintaining high quality for related contents (Sections~\ref{sec:problem-setup} and~\ref{sec:optimization-problem}). 
\item We show that the problem is non-convex, and propose an ADMM-like iterative algorithm that fully exploits the structure of the sequential content access statistics (\secref{sec:optim_algorithm}). %\pavlos{I removed the sentence for the greedy. It didn't make sense to me, and I don't think it's so important to mention, and could not think of a nice way to mention it.}
%We show that the problem is non-convex, consider a myopic algorithm that relates to some existing policies~\cite{chatzieleftheriou2017caching}, and then propose an ADMM-like iterative algorithm that fully exploits the structure of the sequential content access statistics (\secref{sec:optim_algorithm}).
\item Using simulations on a number of real datasets for different content types, we show that our algorithm significantly outperforms baseline approaches and previous work, improving caching performance in a large range of setups, while maintaining the desired recommendation quality (\secref{sec:sims}).
\end{itemize}

As a final note, while in this paper we consider the problem in the simple(r) context of a layer of caches with increasing cost, the proposed approach can be applied on top of a number of the cooperative wireless caching policies discussed earlier, e.g., ~\cite{femto,Ali2014,sermpezis-sch-globecom}. We plan to explore the interplay of such advanced caching policies and the proposed cache-friendly recommender as part of future work.

==> problem_formulation.tex <==


%Having defined in Section~\ref{sec:problem_setup} the generic setup of content access and recommendation, we proceed to formally define the problem of selecting (cache-friendly) recommendations.

%\myitem{The problem.} As discussed above, the content provider aims to (i) minimize the expected content retrieval cost, and (ii) ensure high-quality recommendations. These two goals are of different nature, and thus not directly comparable. While they could be captured in the context of a multi-objective optimization problem, a second challenge is to quantify the quality of recommendations (or, equivalently the user QoE). Without practical evidence and/or experimental deployment, only a worst-case estimation of the quality is possible. 

\begin{comment}
For these reasons, we select to approach the problem using the following formulation: We consider in the optimization objective only the content retrieval cost, and express the need for high-quality recommendations as a constraint (which is in accordance with the ``worst-case'' estimation of quality). Specifically, we define the optimization problem as
\begin{align}\label{eq:opt-words}
\min_{R} &~~\text{Content\_Retrieval\_Cost}\\
&s.t. ~~~\text{High\_Quality\_Recommendations} \nonumber
\end{align}
where the optimization variable $R$ are the recommendations of the RS.

In the following, we first model the content retrieval process and calculate its expected cost (Section~\ref{sec:cost}), and then formulate the constraint for high quality recommendations (Section~\ref{sec:constraint}). We use these results to formulate the optimization problem of cache-friendly recommendations in Section~\ref{sec:optim-problem-formulation}.
\end{comment}

%Given the above setup, our general goal in this paper is \textit{to reduce the total cost of serving user requests by choosing what to recommend based on both the access cost of a content and the content's relevance}.

%\subsection{Content Retrieval Cost}\label{sec:cost}
%Let us consider a user that consumes contents during a viewing session. The session can be split in sequential sub-sessions, each of them starting when the user ignores the recommendations and selects a content from the entire catalogue (which takes place w.p. $1-\alpha$ at each content request).

%\pavlos{IMO this definition should come earlier, in the setup section.} 
%Let us define the recommendation matrix $R$, whose elements $r_{ij}$ are given by \pavlos{in fact, $r_{ij}$ should be defined as the probability that a content is recommended} 
% \begin{equation}
% r_{ij} = \left\{
% \begin{tabular}{ll}
% {1}&{, if $j$ is recommended after $i$}\\
% {0}&{, otherwise}
% \end{tabular}
% \right.
% \end{equation}
%Let us define the recommendation matrix $R$, whose elements $r_{ij}$ indicate whether the content $j$ is recommended after content $i$ ($r_{ij}=1$) or not ($r_{ij}=0$). To generalize this and capture more complex RSs, we define $r_{ij}\in[0,1]$ to be the probability that $j$ is recommended after $i$. Since $N$ contents are recommended after a content $i$, it must hold that
%\begin{equation}
%\sum_{j}r_{ij}=N
%\end{equation}


%\myitem{Modeling the content retrieval process.} 

Our goal in this section is to derive the expected content access cost for a user session, \emph{as a function of the recommendation decisions $R = r_{ij}$}. 

\begin{lemma} Let $S = \{i_{1},i_{2},\dots, i_{s} \}, i_{n} \in \mathcal{K}$ be a sequence of contents accessed by a user during a viewing session. Then $S$ is a Markov chain with transition matrix
\begin{equation}\label{eq:MC}
\mathbf{P} = \frac{\alpha}{N} \cdot \mathbf{R} + (1-\alpha) \cdot \mathbf{p} \cdot \mathbf{1},
\end{equation}
where $\mathbf{1}$ is a column vector of all 1s. 
\end{lemma}
\begin{proof}
When the user has just consumed content $i$, then she might next consume content $j$ if  (a) she decides to follow one of the $N$ recommendation, (b) $j$ is one of the recommended contents, and (c) $j$ is the specific content she chooses out of the $N$ recommended ones. The probability of (a) is $\alpha$, by Def.~\ref{def:user-access}, the probability of (b) is $r_{ij}$, and the probability of (c) is $\frac{1}{N}$. However, the user might also consume $j$ after $i$ if she ignores the recommendations (with probability $1-\alpha$) and picks content $j$ from the entire catalogue (with probability $p_j$). Putting all these together gives the transition probability from $i$ to $j$, $p_{ij} = \frac{\alpha}{N} \cdot r_{ij} + (1-\alpha)\cdot p_j$, which written in matrix notation gives Eq.(\ref{eq:MC}). 
\end{proof}

\begin{lemma}[Content Retrieval Cost]

(a) A user content sequence $S = \{S_{R}^{1},S_{S}^{1},S_{R}^{2},S_{S}^{2},\dots\}$ is an alternating renewal process alternating between  $S_R^{i} = \{i_1,i_2,\dots,i_{R^{i}} \}$, where the user follows recommended contents, and periods $S_S^{i}$, where the user ignores recommendations and picks from the entire catalogue.

(b) The tuple $S,\mathbf{c}$ defines a renewal-reward process, where $c_i$ is the penalty incurred when $S$ visits state $i$. 

(c) Let $C(T)$ denote the total cost of a (sub-)sequence of contents T, $C(T) = \sum_{i\in T} c_{i}$, and $|T|$ denote the length of T. The expected cost per content accessed for a user session $S$ is
\begin{equation}
E[{C(S)}] = \frac{E[C(S_R)] + E[C(S_S)]}{|S_R|+|S_S|}.
\end{equation}
\end{lemma}


We model the content retrieval process during a sub-session with a discrete \textit{absorbing Markov Chain} (AMC). %Given the recommendation matrix $R$, and the fact that a user selects randomly one of the $N$ recommendations w.p. $\alpha$ or ignores them w.p. $1-\alpha$, the content retrieval process during a sub-session can be modeled with a discrete \textit{absorbing Markov Chain} (AMC). 
%
The AMC consists of $K$ transient states that correspond to contents (retrievals) and one absorbing $A$ state that corresponds to the event of a user to ignore all recommendations (i.e., end of the sub-session). After a user consumes a content $i$ (i.e., she is at state $i$) during the sub-session, she then selects to consume another content $j$ (i.e., jumps to state $j$), or ignores the recommendations and leaves the sub-session (i.e., jumps to the absorbing state $A$). We denote the respective transition probabilities as $q_{ij}$ and $q_{iA}$, and calculate them in Lemma~\ref{thm:transition-prob}. 

\begin{lemma}\label{thm:transition-prob}
The transition probabilities of the AMC are given by $q_{ij} = \frac{\alpha}{N} \cdot r_{ij}$ and $q_{iA} = 1-\alpha$.
% \begin{align}
% p_{ij} &= \frac{\alpha}{N} \cdot r_{ij} \label{eq:prob-p-ij}\\
% p_{iA} &= 1-\alpha
% \end{align}
\end{lemma}
\begin{proof}
A user follows a recommendation and retrieve a content $j$, after consuming content $i$, when all the following conditions hold: (i) the user follows a recommendation, (ii) content $j$ is recommended, and (iii) the user selects (randomly) $j$ among all recommendations. The probabilities of these events are given by the quantities $\alpha$, $r_{ij}$, and $\frac{1}{N}$, respectively. Since all conditions must hold, multiplying these probabilities, gives the expression for $q_{ij}$. The probability $q_{iA}$ follows directly from the model.
\end{proof}



\myitem{Calculating the expected content retrieval cost.} We first calculate the \textit{total} expected cost of content retrievals during a sub-session (Lemma~\ref{thm:total-cost-sub-session}), and then apply the renewal-reward theory to calculate the expected cost per content retrieval in a session  (Theorem~\ref{thm:expected-cost}). 



\begin{lemma}\label{thm:total-cost-sub-session}
The total expected content retrieval cost during a sub-session is given by
\begin{equation}\label{eq:total-cost-sub-session}
E[C_{sub-session}] = \mathbf{p}^{T}\cdot F \cdot \mathbf{c}
\end{equation}
where %$\mathbf{p}$ and $\mathbf{x}$ the content \rem{probability} and cost vectors, respectively, and
\begin{equation}\label{eq:fundamental-matrix-expression}
F = \left(I - \frac{a}{N}\cdot R \right)^{-1}
\end{equation}
and $P=\mathbf{p}\cdot \mathbf{1}^{T}$, and $\mathbf{1} = [1,1,...,1]^{T}$ the unit vector of size $K\times 1$, and $I$ the identity matrix of size $K\times K$.
\end{lemma}
\begin{proof}
Let a user start a sub-session by retrieving content $i$. The expected number of retrievals of content $j$ (or, number of times visiting state $j$) until the end of the sub-session is given by $f_{ij}$, where $f_{ij}$ is the ($i$-row,$j$-column) element of the \textit{fundamental matrix} $F$ of the AMC\pavlos{ref?}.

The fundamental matrix is defined as 
\begin{equation}\label{eq:fundamental-matrix-definition}
F = \sum_{n=0}^{\infty} Q^{n} = (I-Q)^{-1}
\end{equation}
where $Q$ the matrix with the transition probabilities $q_{ij}$ between the transient states of the AMC ($i,j\in\mathcal{K}$). From Lemma~\ref{thm:transition-prob}, we have that $q_{ij} = \frac{\alpha\cdot r_{ij}}{N}$, thus, we can write for the matrix $Q$
\begin{equation}\label{eq:transient-matrix}
Q = \frac{\alpha}{N}\cdot R
\end{equation}
Substituting \eq{eq:transient-matrix} in \eq{eq:fundamental-matrix-definition} gives the expression of \eq{eq:fundamental-matrix-expression}.

Now, the cost of retrieving a content $j$ is $c_{j}$. Since each content $j$ is retrieved on average $f_{ij}$ times during a sub-session that starts from $i$, the total cost is given by 
\begin{equation}
E[C_{sub-session}~|~ i] = \sum_{j\in\mathcal{K}} f_{ij}\cdot x_{j}
\end{equation}
The probability that a sub-session starts at content $i$ is equal for all sub-sessions and is given by $p_{i}$. Thus, taking the expectation over all the possible initial states $i$, gives
\begin{equation}
E[C_{sub-session}] = \sum_{i\in\mathcal{K}} E[C_{sub-session}~|~ i] \cdot p_{i} =  \sum_{i\in\mathcal{K}} \sum_{j\in\mathcal{K}} f_{ij}\cdot c_{j} \cdot p_{i}
\end{equation}
Expressing the above summation as the product of the vectors $\mathbf{p}$ and $\mathbf{x}$, and the matrix $F$, gives the expression of \eq{eq:total-cost-sub-session} for the total expected cost during a sub-session.
\end{proof}


\begin{theorem}\label{thm:expected-cost}
The expected cost per content retrieval in a session is given by
\begin{equation}
E[C] = (1-\alpha)\cdot \mathbf{p}^{T}\cdot F \cdot \mathbf{c}
\end{equation}
\end{theorem}
\begin{proof}
Let a session composed of $M$ sub-sessions, and in each sub-session $m$, $m=1,...,M$, a user retrieved $W_{m}$ contents, whose total cost is $EC_{m}$. Then, the average cost per content retrieval for the entire session is given by
\begin{equation}
C = \frac{\sum_{m=1}^{M}C_{m}}{\sum_{m=1}^{M}W_{m}}
\end{equation}
\pavlos{renewal theory happens here and we can write the above as...}
\begin{equation}\label{eq:expectation-ratio-expectations}
E[C] = \frac{E[C_{sub-session}]}{E[W_{sub-session}]}
\end{equation}
where $E[C_{sub-session}]$ denotes the expected total cost per sub-session and $E[W_{sub-session}]$ is the average number of content retrievals per sub-session. The former quantity can be calculated by Lemma~\ref{thm:total-cost-sub-session}. For the latter, we proceed as follows: After consuming a content, a user stays in the sub-session w.p. $\alpha$ or leaves it w.p. $1-\alpha$. We can describe this with a Bernoulli process where a ``success'' denotes the end of the sub-session, and takes place w.p $1-\alpha$. Therefore, the number of contents retrievals $W_{m}$ in a session is given by a geometric distribution with rate $1-\alpha$. The average number of a geometric distribution with rate $t$ is $\frac{1}{t}$ \rem{[cite]} and thus the average number of content retrievals during a sub-session is
\begin{equation}\label{eq:expected-nb-steps}
E[W_{sub-session}]=\frac{1}{1-\alpha}
\end{equation}

Substituting the expressions of Lemma~\ref{thm:total-cost-sub-session} and \eq{eq:expected-nb-steps}, in \eq{eq:expectation-ratio-expectations} proves the theorem.
\end{proof}

% Consider a user that starts a session by requesting a content $i\in\mathcal{K}$ with probability $s_{i}$ (i.e., we assume her initial choice is not affected by the recommender). The user then proceeds to request a sequence of contents according to the Markov chain $P$ of Eq.(\ref{eq:Google-Markov-Matrix}). Assume that the user requests $M$ contents in sequence. Then the associated access cost would be given by
% \begin{equation}\label{cost-finite-steps}
% \sum_{m=0}^{M} \mathbf{p_0}^{T}\cdot P^{m} \cdot \mathbf{x},
% \end{equation}
% where $\mathbf{x} = [x_{1},...,x_{K}]^{T}$ is the vector of the costs per content (see \secref{sec:problem-setup}).

% $M$ is a random variable though, and the various powers of transition matrix $P$, which contains the control variable $Y$, would greatly complicate the problem. However, the above Markov chain is strongly connected and ergodic under very mild assumptions for $\mathbf{p_0}$. It thus has a stationary distribution $\boldsymbol{\pi} = [\pi_{1},...,\pi_{K}]^{T}$, which is also equal to the long-term percentage of total requests for content $i$. Consequently, for $M$ large enough we can approximate the average cost \textit{per request} with
% \begin{equation}\label{eq:definition-average-cost}
% \boldsymbol{\pi}^{T}\cdot \mathbf{x}
% \end{equation}
% where $\boldsymbol{\pi}$ can be calculated from the following lemma.

% \begin{lemma}\label{lemma:stationary-analytical-expression}
% The stationary distribution $\boldsymbol{\pi}$ is given by
% \begin{equation}\label{eq:stationary-analytical-expression}
% \boldsymbol{\pi}^{T} = (1-a)\cdot  \mathbf{p_0}^{T} \cdot (I - a\cdot Y)^{-1} 
% \end{equation}
% where $I$ the $K\times K$ identity matrix.
% \end{lemma}
% \begin{proof}
% The stationary distribution above can be derived through the standard stationary equality~\cite{mor2013}
% \begin{equation}
% \boldsymbol{\pi}^{T} =a \cdot \boldsymbol{\pi}^{T} \cdot Y + (1-a) \cdot  \mathbf{p_0}^{T}, 
% \end{equation}
% by observing that matrix $(I - a\cdot Y)$ has strictly positive eigenvalues (in measure). See also~\cite{avrachenkov2006pagerank}, for more details.
% \end{proof}




\subsection{High Quality Recommendations}\label{sec:constraint}
A content $j$ is recommended after content $i$ with probability $r_{ij}$, and a ``worst-case'' estimation for the quality of recommending $j$ after $i$ is given by their score $u_{ij}$. Therefore, the (expectation of the) total quality of recommendations for $i$ is at least $\sum_{j\in\mathcal{K}} r_{ij}\cdot u_{ij}$, and a RS aiming to provide high quality recommendations, should require that this sum is always larger than a minimum threshold, let $q_{i}$, i.e.,
\begin{equation}\label{eq:constraint-definition}
\sum_{j\in\mathcal{K}} r_{ij}\cdot u_{ij} \geq q_{i}
\end{equation}


For a content $i$, if we denote the vectors of its scores with every other content as $\mathbf{u_{i}} = [u_{i1}, ..., u_{iK}]^{T}$. Assuming w.l.o.g. that $u_{i1}>u_{i2}>...>u_{iK}$, the maximum quality that can be achieved in a list of $N$ recommendations is $\sum_{j=1}^{N}u_{ij}$. Hence, the threshold $q_{i}$ can take values in the range $[0,\sum_{j=1}^{N} u_{ij}]$. The largest the value of $q_{i}$. The less flexible the choice of recommendations; e.g., for $q_{i}=\sum_{j=1}^{N} u_{ij}$ there is only one set of contents that can be recommended, while for $q_{i}=0$, any set of $N$ contents can be recommended.

In the remainder, we assume the threshold $q_{i}$ is given, and is set by the RS to a desired value.

\subsection{Optimization Problem}\label{sec:optim-problem-formulation}
Applying in the problem described in \eq{eq:opt-words}, Theorem~\ref{thm:expected-cost} for the objective function and \eq{eq:constraint-definition} for the constraint, leads to the formulation of the Optimization Problem~\ref{problem:basis}.

\begin{problem}[Cache-Friendly Recommendations]\label{problem:basis}
\begin{small}
\begin{subequations}\label{eq:objective-infinite-step}
\begin{align}
\underset{\mathbf{R}}{\mbox{minimize}} \; \; \; \; & 
  (1-\alpha)\cdot \mathbf{p}^{T}\cdot \left(I - \frac{a}{N}\cdot \mathbf{R} \right)^{-1} \cdot \mathbf{c}, \tag{\ref{eq:objective-infinite-step}}\\
& \sum_{j =1}^{K}   r_{ij} u_{ij} \geq q_i, ~~\forall i~\in \mathcal{K},
\label{quality-con}\\
& \sum_{j = 1}^{K}   r_{ij} = N, ~~\forall i~\in \mathcal{K} \label{affine-con}\\
&    r_{ij} \begin{cases} 
      \in \big[0,1 \big], & \text{if}\ i \neq j \\
      = 0, & \text{otherwise}
    \end{cases}~~~\forall i,j\in\mathcal{K} \label{box-con}
\end{align}
\end{subequations}
\end{small}
\end{problem}%
%
where (i) in the objective, we used the expression of \eq{eq:fundamental-matrix-expression} for the fundamental matrix $F$, and (ii) included also the required constraints (see \pavlos{definition of $r_{ij}$}) for the recommendation variables in \eq{affine-con} and \eq{box-con}.

\myitem{Problem characteristics.} The problem comprises $K^{2}$ variables $r_{ij}$, and a set of $K^{2}+2\cdot K$ linear (equality and inequality) constraints. The objective function involves an inverse matrix of the variables\rem{, and in the general case it is non-convex.} \pavlos{???} In the following section, we propose an algorithm to approximately solve the Optimization Problem~\ref{problem:basis}.



% We are therefore ready to formulate cache-friendly recommendations as an optimization problem.

% \begin{problem}[Cache-Friendly Recommendations]\label{problem:basis}
% \begin{small}
% \begin{subequations}\label{eq:objective-infinite-step}
% \begin{align}
% \underset{Y}{\mbox{minimize}} \; \; \; \; & 
%   p_{0}^{T} \cdot (I-aY)^{-1} c, \tag{\ref{eq:objective-infinite-step}}\\
% & \sum_{j = 1}^{K}   y_{ij} = 1, ~~\forall i~\in \mathcal{K} \label{affine-con}\\
% & \sum_{j =1}^{K}   y_{ij} u_{ij} \geq q_i, ~~\forall i~\in \mathcal{K},
% \label{quality-con}\\
% &    y_{ij} \begin{cases} 
%       \in \big[0,\frac{1}{N} \big], & \text{if}\ i \neq j \\
%       = 0, & \text{otherwise}
%     \end{cases} \label{box-con}
% \end{align}
% \end{subequations}
% \end{small}
% \end{problem}

% \myitemit{Objective.} The objective is to minimize the expected cost to access any content, and follows directly from \eq{eq:definition-average-cost} and Lemma~\ref{lemma:stationary-analytical-expression}. Note that we have dropped the constant $(1-a)$ from \eq{eq:stationary-analytical-expression}, as it does not affect the optimal solution. 

% \myitemit{Control Variables.} The variables $y_{ij}$ ($K^{2}$ in total), deciding what is recommended after each content $i$, constitute the control variables. 

% \myitemit{Constraints.} The first three constraints make sure that $y_{ij}$ forms a stochastic transition matrix that can be translated to $N$ recommendations per item $i$. Specifically, the ``box'' constraints of \eq{eq:y-box-constraint} ensures that all entries are positive, and smaller or equal to $1/N$. The latter is necessary as matrix $Y$ is a \textit{normalized} version of the recommendations. Together with \eq{eq:sum-y-equals-1-constraint} these ensure that exactly $N$ contents are recommended for every $i$ (see also Section~\ref{sec:problem-setup}, ``Recommendation Control''). \eq{eq:no-self-recommendations-constraint} simply ensures that the same content cannot be recommended when it was just consumed.

% \myitemit{Quality Constraint.} \eq{eq:quality-constraint} ensures that that the ``quality'' of recommended contents for each $i$ is above a desired threshold. Observe that, without this constraint, the optimal solution to the above problem is trivial, namely to always recommend the same $N$ contents $j$ with the minimum cost $x_{j}$. However, these contents will probably be unrelated (i.e. $u_{ij} \rightarrow 0$) essentially ``breaking'' the recommender. Hence, this constraint forces variables $y_{ij}$ to select high $u_{ij}$ values to ensure the recommender keeps doing its primary job, namely finding related contents. Note that, if there are at least $N$ strongly related contents for each $i$ (i.e., $u_{ij} = 1$), then the maximum value for $q_i$ is $1$. W.l.o.g., in the remainder we will assume the same quality constraint for all $i$ ($q_i = q$). 

% The remaining quantities are constants, and inputs to the problem. While some of them might still vary over time (e.g., $u_{ij}$), we assume this occurs at a larger time scale, compared to our problem.



==> todolist.tex <==
\begin{enumerate}

%\item List of things that could be shrunk if final text is more than 9 pages: (i) text of list of contributions; (ii) Lemma 3's proof; (iv) the "win-win" scenario in Section 2.; (v) proof of Lemma 2.

%\item \purple{Write the convergence lemma for after the algorithm. PAEI}

%\item purple{Write the tech report latex. The tech report should contain: (i) the proofs for the 3 inequalities (for the main theorem); (ii) the proof of fast greedy (probably), (iii) the proof of Lemma 7(?)...convergence of subroutines, (iv) a few more plots ON GOING (v) Lemma and proof Greedy (0-1 cost, generic u)}

%\item Notation table; add any variable that you use more twice. also, there's a couple inconsistencies.

%\item Liakopoulos ``extreme'' shrinking toolkit.

%\item replace Q (quality) with q. (in captions too!!!!)

%\item Update the captions of figures. PAEI

%\item Include lastfm, Youtube Pavlos (more), and movielens. PAEI

%\item \purple{Include an execution time comparison admm-cvx vs admm-(gradient+projections) (tha to valw inline sto keimeno)}

%\item \purple{Make sure that everything in the figures (captions, legends, axes, etc., containt the correct notation and terms, from the new version)}

%\item create an anonymous tech report to see how it's done. \add{AND ADD THE TECH REPORT TO THE CITATIONS. FIX ALSO ALL REFERENCES TO THIS TECH REPORT}

\item include the (baseline) cache hit rate for the "most popular" policy to each scenario; just put it inline in the text; 

%\item replace fig.3b (last.fm with respect to q) with last.fm with respect to alpha (e.g. values 0.5 to 0.9) with a high q value (e.g. 85 or 90\% where we are quite better than greedy)

%\item fix the convergence plot as I suggested.

\item Generalize quality constraint: I mean to show that we could also have a "weighted" quality constraint of type $sum_j n_{ij} \cdot u_{ij}$ ($n_{ij}$ coming from the fundamental matrix. this weighs in how often a user sees an item $j$, while our original is more ``fair'' content-wise (we need a good quality for ALL contents, not just the frequently visited ones). I would add this in the discussion.

%\item Related Work section

%\item Search for ADMM convergence rate proofs/results. AND add missing references about why ADMM and not LP (Very important!)

%\item define the probability $p^{K\prime}$ (probably as $P_{shrink}$) inside Lemma 9, right after Eq.(20). Then use that notation in your plots and text descriptions.

%\item update all the theory for correct/new quality constraint 

%\item shorten abstract

%\item avoid referring to our algorithm as "ADMM" too much (for reasons I mentioned)

%\item fix notation inconsistencies about F.

%\item fix notation inconsistencies about $p_0$ (see def.1)

%\item Prove the last part of the fast-greedy scheme.

%\item fill in all missing references

\item a plot to compare with the paper that introduces irrelevant but cached elements in the list.

%\item check the ICASP paper (or other ones) to see if the implement inner loops with CVX minimization. This way we don't have to only refer to our previous work.

\item add figure fig:AMC in Section III, showing a sequence of recommendation and teleport periods and its relation to the absorbing markov chain.\pavlos{done}

\item Discussion and Conclusions: topics to discuss potentially: (i) implementation (where by whom?), (ii) joint caching and recommendation (ACS and 1 plot?), (iii) dynamic learning of $\alpha$ and other parameters (OCO, Q-learning), (iv) follow recommendations with prob. different than $1/N$ (e.g., based on position).\pavlos{I added these in conclusions}

\item check Infocom email about pdf format. \add{try it TONIGHT, to make sure you know how to do}

\item Recommendation driven cost: if we need space, this lemma can probably be reduced.

%\pavlos{IMPORTANT: i noticed we have $\mathbf{z}^T - \frac{\alpha}{N} \mathbf{z}^{T}\cdot\mathbf{R} = \boldsymbol{p}_0^T$ after that we make the change of variables we say $\mathbf{z}^T \mathbf{R} = \mathbf{1}^T\mathbf{F}$ which is now wrong. So I will go wherever $f_{ij}$ appears as a scalar and redefine it as $f_{ij} = \frac{\alpha}{N} z_i \cdot r_{ij}$-did it check if you see anything stravo}

\pavlos{Check from the TWO youtube papers cache recommendation if you refer to the correct one}

\pavlos{We need to change the gains written in the abstract, especially since we wont present lastfm which displays the largest gain (about 100\% in q=1}

\item \add{IMPORTANT: update title and abstract in EDAS}
\end{enumerate}
